Secure and User-Friendly Over-the-Air Firmware Distribution in a Portable Faraday Cage

Setting up a large-scale wireless sensor network is challenging, as firmware must be distributed and trust between sensor nodes and a backend needs to be established. To perform this task efficiently, we propose an approach named Box, which utilizes an intelligent Faraday cage (FC). The FC acquires firmware images and secret keys from a backend, patches the firmware with the keys and deploys those customized images over the air to sensor nodes placed in the FC. Electromagnetic shielding protects this exchange against passive attackers. We place few demands on the sensor node, not requiring additional hardware components or firmware customized by the manufacturer. We describe this novel workflow, implement the Box and a backend system and demonstrate the feasibility of our approach by batch-deploying firmware to multiple commercial off-the-shelf sensor nodes. We conduct a user-study with 31 participants with diverse backgrounds and find, that our approach is both faster and more user-friendly than firmware distribution over a wired connection.

==> Problem_Statement.tex <==
\section{Adversarial Model}
\label{Sec:ProblemStatement}
The goal of the attacker is to be able to eavesdrop the firmware and key exchange between Box and sensor nodes from outside the Box.
%
We assume the attacker to be present before, during and after firmware distribution.
%
He is computationally bounded, implying that his computing power is polynomial at most.
%
%WIRELESS AKTIV----------------------------------------
%The attacker can eavesdrop, replay and modify any message transmitted and inject arbitrary messages.
%%
%Further, he can jam the wireless channel on the physical and upper layers or delay messages in order to launch a denial of service attack.


%PHYSICAL----------------------------------------
We assume that the attacker neither has physical access to the backend, nor to the Box.
%%
%He is able to capture sensor nodes before and after deployment, extract firmware and write new firmware to those.
%%
%If a node is compromised, all information stored in its memory must be considered compromised.
%
%
The operator of the box is assumed trustworthy and aware of his surroundings, i.e.~able to notice obviously strange events.




%SUPPLY CHAIN------------------------------------
%We assume, that the device manufacturer who deploys the \gls{OTA} bootloader does not insert any undesired functionality.
%
%This is a reasonable assumptions, as an untrusted device manufacturer could manipulate hardware as well, undermining security of all layers above.
%

%OLD STUFF
%This, however not stated explicitly, is done by all comparable solutions. %, as this would render them pointless.
%%
%Either, they assume that firmware was deployed to the device \textit{somehow} prior to key distribution.
%%
%If this is done by a third party, sensor nodes could have firmware backdoors.
%%
%If, however, \gls{WSN} operators deploy firmware themselves, most key distribution approaches from literature are not necessary.
%%
%After all, operators could just place the secret key in the firmware before flashing the sensor node with it, utilizing the physical connection between deploy computer and sensor node as \gls{LLC}.



%We further assume the Backend to be trustworthy.
%%
%We assume the network to operate such that sensor nodes send data, destined to an application at the Backend.
%%
%Thus, we require end to end encryption and authentication between sensor node and Backend.
%%
%Sensor nodes do not need to contact each other.
%%
%If a multi-hop (mesh) network topology is chosen, intermediate sensor nodes can neither eavesdrop nor modify the traffic they relay.

==> Related_Work.tex <==
\section{Related Work}
\label{Sec:RelatedWork}
Many \gls{LLC} channels have been proposed, such as visual channels, where devices exchange secrets or authentication information using visible \cite{Saxena2006, Saxena2009, Gauger2009} or invisible light
%
% \cite{Feeney2002, Saxena2006, Saxena2008, Saxena2008a, Roth2008, Saxena2009, Gauger2009, Perkovic2009, Li2010, Saxena2011, Perkovic2012, Kovacevic2013, Kovacevic2016} or invisible light 
%
\cite{Balfanz2002, Balfanz2004}, 
%\cite{Balfanz2002, Swindells2002, Rekimoto2003, Balfanz2004}, 
%laser \cite{Kindberg2003}, 
flashing smart phone displays \cite{Kovacevic2016} or QR Codes \cite{McCune2005, Das2017}.
%
Audio channels have also been proposed frequently
\cite{Lopes2001, Goodrich2006, Soriente2008}.
%\cite{Lopes2001, Kindberg2003a, Goodrich2006, Saxena2008a, Soriente2008}.

The human operator can be considered a \gls{LLC}, inserting data into devices by shaking devices together \cite{Holmquist2001, Lester2004, Castelluccia2005, Mayrhofer2007}
%
%\cite{Holmquist2001, Lester2004, Castelluccia2005, Mayrhofer2007, Mayrhofer2009}
%
, pointing a provisioning device \cite{Swindells2002, Hoepman2008} or entering keys \cite{Bluetooth5Specification}.
%
The operator can also be tasked to compare data displayed at two devices \cite{Cagalj2006, Prasad2008, Chen2008, Li2010, Perkovic2012, Bluetooth5Specification} 
%\cite{Li2013, }
or relay data \cite{Gehrmann2004, Soriente2007,  Bluetooth5Specification}.
%
Using the human body as transmission channel can be considered a flavor of relay data \cite{Venkatasubramanian2010, Hu2013, Roeschlin2018} and is mainly used in \glspl{BAN}.
%
We do not consider \gls{LLC} approaches related to our Box, as all of those utilize additional hardware at the sensor node to create a \gls{LLC}.



The idea to use a \gls{FC} to create a \gls{LLC} has been mentioned in one sentence by Castelluccia and Mutaf \cite{Castelluccia2005}.


%KUO ET AL
Kuo \etal are the first to implement this approach and show, that exchanging pairwise keys between a base station and sensor nodes in a \gls{FC} has high usability \cite{Kuo2007}.
%
Their approach is limited by the requirement, that simultaneous bootstrapping of multiple sensor nodes is only possible if they are of the same type.
%
Additionally, their protocol needs to be implemented in the firmware of every sensor node.
%
This firmware must be delivered to sensor nodes by some unspecified means, so one could argue, that keys could just have been transferred with the firmware image over the same wired connection.
%
Our approach overcomes this issue by utilizing the \gls{OTA} firmware distribution with embedded keys, keeping all functions needed for firmware and key exchange into the \gls{OTA} bootloader.
%
By having this split of responsibilities, our runtime firmware can be kept small, maximizing reliability and thus sensor node availability.
%
Further, our Box approach permits mixing different sensor nodes as needed while distributing firmware.


To reduce the \gls{SNR} at the attacker, Kuo \etal use a jammer attached at the exterior of the Faraday cage \cite{Kuo2007}.
%
While this is beneficial to increase security levels, jamming power must adhere to regulations.
%
Further, benign nearby devices might be jammed, too, decreasing their availability.
%
Our approach does not need a jammer, as we introduce a combination of software and chained hardware attenuators to reduce the transmission power inside the Box to a low level.
%
This, in addition with the shielding, results in a low \gls{SNR}, effectively preventing eavesdropping by an external attacker. 
%
\msr{Mixed node support? Dann hinschreiben, wenn ich es an der anderen Stelle sauber ergänzt habe.}

We consider our approach a leap towards real-world applicability, reducing the number of hardware parts needed, not interfering with nearby devices and especially solving the issue of initial firmware distribution, which was previously assumed to happen implicitly.





%LAW ET AL
Law et al.~use \gls{ECDH} key exchange inside a \gls{FC} \cite{Law2011}.
%
Sensor nodes then create a body sensor network.
%
While public key cryptography is beneficial in terms of key management, it creates high demands on the computational performance of a sensor node.
%
Furthermore, they require that a sensor node can generate pseudo-random numbers with sufficient entropy as well as a jammer attached to the \gls{FC}.
%
Unlike our approach, they require the user to make security-critical decisions by forcing her to configure the \gls{FC}.
%
In comparison, our approach is easier to follow and thus less error-prone, as we do not need dedicated protocols for initial deployment and node addition, which in Law's approach forces the user to follow different workflows.
%
%Need keep-alive packets authenticated and fresh to prevent that a captured node reveals group global keys.}
